Hybrid Computing for Interactive Datacenter Applications

Field-Programmable Gate Arrays (FPGAs) are more energy efficient and cost effective than CPUs for a wide variety of datacenter applications. Yet, for latency-sensitive and bursty workloads, this advantage can be difficult to harness due to high FPGA spin-up costs. We propose that a hybrid FPGA and CPU computing framework can harness the energy efficiency benefits of FPGAs for such workloads at reasonable cost. Our key insight is to use FPGAs for stable-state workload and CPUs for short-term workload bursts. Using this insight, we design Spork, a lightweight hybrid scheduler that can realize these energy efficiency and cost benefits in practice. Depending on the desired objective, Spork can trade off energy efficiency for cost reduction and vice versa. It is parameterized with key differences between FPGAs and CPUs in terms of power draw, performance, cost, and spin-up latency. We vary this parameter space and analyze various application and worker configurations on production and synthetic traces. Our evaluation of cloud workloads shows that energy-optimized Spork is not only more energy efficient but it is also cheaper than homogeneous platforms--for short application requests with tight deadlines, it is 1.53x more energy efficient and 2.14x cheaper than using only FPGAs. Relative to an idealized version of an existing cost-optimized hybrid scheduler, energy-optimized Spork provides 1.2-2.4x higher energy efficiency at comparable cost, while cost-optimized Spork provides 1.1-2x higher energy efficiency at 1.06-1.2x lower cost.

==> figures/motivation/ilp_scheduler.tex <==
\section{ILP Formulation}
\label{sec:ilp_scheduler}

Rate-based ILP scheduler; tries to match input and output processing rates and
minimizes overall energy use.

\medskip
\noindent\textbf{Assumptions:}

\begin{itemize}
	\item Functions with fully known load
	\item All functions have same energy usage characteristics
	\item (De)allocations are instantaneous, but still cost energy
	\item Arriving requests are available at start of their time interval
	\item Requests complete within the time interval they arrive in
	\item Deadlines are always met
\end{itemize}

\medskip
\noindent\textbf{Inputs:}

$X_{j,t} \in [0, \infty)$: number of requests that arrive for function $j$ in time $[t, t+1)$

$e^{c}_{b}, e^{f}_{b}$ : busy power consumption of CPU, FPGA

$e^{c}_{i}, e^{f}_{i}$ : idle power consumption of CPU, FPGA

$a^{c}, a^{f}$: allocation energy of CPU, FPGA

$d^{c}, d^{f}$: deallocation energy of CPU, FPGA

$r^{c}, r^{f}$ : request processing rate of CPU, FPGA

\medskip
\noindent\textbf{Outputs:}

$Y^{c}_{j,t} \in [0, N_{cpu}]$: total CPUs allocated to function $j$ at time $t$

$Y^{f}_{j,t} \in [0, N_{fpga}]$: total FPGAs allocated to function $j$ at time $t$

$B^{c}_{j,t}, B^{f}_{j,t} \in [0, N_{r}]$: busy CPUs, FPGAs of function $j$ at time $t$

\medskip
\noindent\textbf{Helpers:}

$I^{c}_{j,t}, I^{f}_{j,t} \in [0, N_{r}]$: idle CPUs, FPGAs of function $j$ at time $t$

$E^{a}_{t}$: total allocation energy consumed at time $t$

$E^{b}_{t}$: total energy consumed at time $t$ for busy resources

$E^{i}_{t}$: total energy consumed at time $t$ for idle resources

$E^{d}_{t}$: total deallocation energy consumed at time $t$

\medskip
\noindent\textbf{Optimization:}

$\min \sum_{j,t}(E^{a}_{j,t} + E^{b}_{j,t} + E^{i}_{j,t} + E^{d}_{j,t})$

such that,

$\forall j,t: E^{a}_{j,t} = \sum_{r\in{c, f}}\max(Y^{r}_{j,t+1} - Y^{r}_{j,t}, 0) a^r$
: total allocation energy over both resources

$\forall j,t: E^{b}_{j,t} = \sum_{r\in{c, f}} e^{r}_{b}B^{r}_{j,t}$
: total busy energy over both resources

$\forall j,t: E^{i}_{j,t} = \sum_{r\in{c, f}} e^{r}_{i}I^{r}_{j,t}$
: total idle energy over both resources

$\forall j,t: E^{d}_{j,t} = \sum_{r\in{c, f}}\max(Y^{r}_{j,t} - Y^{r}_{j,t+1}, 0) d^r$
: total deallocation energy over both resources

$\forall j,t: r^{c}B^{c}_{j,t} + r^{f}B^{f}_{j,t} \geq X_{j,t}$
: total busy capacity exceeds inputs requests for each function

$\forall j,t: Y^{c}_{j,t} = B^{c}_{j,t} + I^{c}_{j,t}$
: total allocated CPUs is busy + idle

$\forall j,t: Y^{f}_{j,t} = B^{f}_{j,t} + I^{f}_{j,t}$
: total allocated FPGAs is busy + idle

$\forall t: \sum_{j} Y^{c}_{j,t} <= N_{cpu}$
: bound total allocated CPUs

$\forall t: \sum_{j} Y^{f}_{j,t} <= N_{fpga}$
: bound total allocated FPGAs

==> misc/packages.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SPACE SAVERS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\RequirePackage[small,compact]{titlesec}
%%% left, before, after
%\titlespacing*{\section}{0pt}{3pt}{0pt}
%\titlespacing*{\subsection}{0pt}{2pt}{0pt}
%\textfloatsep 0.08in
%\floatsep 0.06in

%%% PATCH TO FIX NUMBERING (titlesec bug removes numbering)
% https://tex.stackexchange.com/questions/299969/titlesec-loss-of-section-numbering-with-the-new-update-2016-03-15
%\RequirePackage{etoolbox}
%\makeatletter
%\patchcmd{\ttlh@hang}{\parindent\z@}{\parindent\z@\leavevmode}{}{}
%\patchcmd{\ttlh@hang}{\noindent}{}{}{}
%\makeatother

%%% AMSMATH (align*) SPACING
%\expandafter\def\expandafter\normalsize\expandafter{%
%  \normalsize
%  \setlength\abovedisplayskip{1pt}
%  \setlength\belowdisplayskip{1pt}
%  \setlength\abovedisplayshortskip{1pt}
%  \setlength\belowdisplayshortskip{1pt}
%}

\def\Section {\S}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% PACKAGES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\RequirePackage{algorithm}
\RequirePackage[noend]{algpseudocode}
\newcommand{\algorithmautorefname}{Algorithm}
\RequirePackage{amsmath}
\RequirePackage{amsthm}
\RequirePackage{amsfonts}
\RequirePackage{array}
\RequirePackage{booktabs}
\RequirePackage{boxedminipage}
\RequirePackage{calrsfs}
\RequirePackage{caption}
\RequirePackage{color}
\RequirePackage{enumitem}
\RequirePackage{fancyhdr}
\RequirePackage{float}
\RequirePackage{graphicx}
\RequirePackage{xcolor}
%\RequirePackage{hyperref}
%\hypersetup{
%	unicode=true,
%    bookmarksnumbered=true,
%	%pdfstartview={FitH},
%	colorlinks=true,
%	linkcolor={red!70!black},
%	citecolor={red!70!black},
%	urlcolor={blue!70!black},
%	pdfborder={0 0 0}
%}
\RequirePackage[capitalize,nameinlink]{cleveref}
\makeatletter
\newcommand{\crefnames}[3]{%
  \@for\next:=#1\do{%
    \expandafter\crefname\expandafter{\next}{#2}{#3}%
  }%
}
\makeatother
\crefnames{part,chapter,section}{\S}{\S\S}
\Crefformat{figure}{#2Fig.~#1#3}
\Crefmultiformat{figure}{Figs.~#2#1#3}{ and~#2#1#3}{, #2#1#3}{ and~#2#1#3}
\Crefformat{algorithm}{#2Alg.~#1#3}
\Crefmultiformat{algorithm}{Algs.~#2#1#3}{ and~#2#1#3}{, #2#1#3}{ and~#2#1#3}
\Crefformat{equation}{#2Eq.~#1#3}
\Crefmultiformat{equation}{Eqs.~#2#1#3}{ and~#2#1#3}{, #2#1#3}{ and~#2#1#3}
\RequirePackage[T1]{fontenc}
\RequirePackage[utf8]{inputenc}
\RequirePackage{listings}
\RequirePackage{microtype}
\microtypecontext{spacing=nonfrench}
\RequirePackage{multirow}
\RequirePackage{nicefrac}
\RequirePackage{pifont}
\RequirePackage[section]{placeins}
\RequirePackage{sidecap}
\RequirePackage{subcaption}
\RequirePackage{url}
\RequirePackage{verbatim}
\RequirePackage{xspace}
\RequirePackage{framed}
\RequirePackage{tcolorbox}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% BIBLIOGRAPHY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\RequirePackage[backend=biber,style=acmnumeric,datamodel=acmdatamodel,autocite=plain,sortcites=true,url=false,maxbibnames=99,date=year]{biblatex}
\RequirePackage[backend=biber,style=acmnumeric,datamodel=acmdatamodel,autocite=plain,sortcites=true,url=false,maxbibnames=99,date=year]{biblatex}
\renewbibmacro{in:}{}
\addbibresource{paper.bib}
\DeclareLabeldate[online]{%
  \field{date}
  \field{year}
  \field{eventdate}
  \field{origdate}
}
\renewbibmacro*{year}{%
  \iffieldundef{year}%
    {}% We omitted the default value "[n. d.]" of ACM here!
    {\printfield{year}}%
}
\DeclareFieldFormat*{eventtitle}{\textit{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SETTINGS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\lstset{
	%language=HTML,
	%basicstyle=\scriptsize\ttfamily,       % the size of the fonts that are used for the code
	basicstyle=\footnotesize\ttfamily,       % the size of the fonts that are used for the code
	%numbers=left,                   % where to put the line-numbers
	numbers=none,                   % where to put the line-numbers
	numberstyle=\scriptsize,        % the size of the fonts that are used for the line-numbers
	stepnumber=1,                   % the step between two line-numbers. If it is 1 each line will be numbered
	numbersep=5pt,                  % how far the line-numbers are from the code
	backgroundcolor=\color{white},  % choose the background color. Add \RequirePackage{color}
	showspaces=false,               % show spaces adding particular underscores
	showstringspaces=false,         % underline spaces within strings
	showtabs=false,                 % show tabs within strings adding particular underscores
	frame=none,                     % adds a frame around the code
	tabsize=2,                      % sets default tabsize to 2 spaces
	captionpos=b,                   % sets the caption-position to bottom
	breaklines=true,                % sets automatic line breaking
	breakatwhitespace=false,        % sets if automatic breaks should only happen at whitespace
	escapeinside={\%*}{*)},         % if you want to add a comment within your code
	commentstyle=\color{green},
	keywordstyle=\color{blue}\bfseries,
	stringstyle=\color{red}
}
\lstdefinelanguage{javascript}{
	keywords={typeof, new, true, false, catch, function, return, null, catch, switch, var, if, in, while, do, else, case, break},
	keywordstyle=\color{blue}\bfseries,
	ndkeywords={class, export, boolean, throw, implements, import, this},
	ndkeywordstyle=\color{black}\bfseries,
	identifierstyle=\color{black},
	sensitive=false,
	comment=[l]{//},
	morecomment=[s]{/*}{*/},
	commentstyle=\color{purple}\ttfamily,
	stringstyle=\color{red}\ttfamily,
	morestring=[b]',
	morestring=[b]"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% CUSTOM COMMANDS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\squishlist}{\begin{itemize}[itemsep=0pt,parsep=0pt,topsep=0pt,partopsep=0pt,leftmargin=1em,labelwidth=1em,labelsep=0.5em]}
		\newcommand{\squishlistend}{\end{itemize}}
\newcommand{\squishend}{\end{itemize}}
\newcommand{\squishenum}{\begin{enumerate}[itemsep=0.5pt,parsep=0pt,topsep=0pt,partopsep=0pt,leftmargin=1.5em,labelwidth=1em,labelsep=0.5em]{}}
		\newcommand{\squishenumend}{\end{enumerate}}

%\newcommand{\todo}[1]{\textsf{\color{red}{[{TODO: #1}]}}}
%\newcommand{\todo}[1]{[[[{\bf{TODO: #1}}]]]}
\newcommand\myurl[2]{\url{#1}}

\renewcommand{\floatpagefraction}{0.95}

\newcommand{\captionfonts}{\small\bfseries\sffamily}
\makeatletter  % Allow the use of @ in command names
\long\def\@makecaption#1#2{%
	\vskip 0.1in
	\sbox\@tempboxa{{\captionfonts #1: #2}}%
	\ifdim \wd\@tempboxa >\hsize
		{\captionfonts #1: #2\par}
	\else
		\hbox to\hsize{\hfil\box\@tempboxa\hfil}%
	\fi
	\vskip 0in}
\makeatother   % Cancel the effect of \makeatletter

% Theorems
%\newtheorem{mydefinition}{Definition}
%\newtheorem{mytheorem}{Theorem}
%\newtheorem{definition}{Definition}
%\newtheorem{theorem}{Theorem}


==> sections/design.tex <==
\section{\sys Design}
\label{sec:design}

To enable fungible computing at scale, we propose \sys, a resource orchestration
and scheduling framework for disaggregated fungible compute backends. This
section details the target applications and design of the \sys framework.

\subsection{Target Workloads}
\label{sec:target_workloads}

\sys is designed for interactive, user-facing cloud applications that resemble
modern-day latency-sensitive
microservices~\autocite{nadareishvili2016_Microservice,sriraman2020_Accelerometer,martin_Microservices}
and serverless
functions~\autocite{shahrad2020_Serverless,jonas2019_Cloud,wang2018_Peeking,CNCF_serverless}.
Specifically, \sys targets stateless applications that expose well-defined input
and output API and process medium-to-long RPC requests (\textasciitilde10\ms to
a few seconds). Applications can be invoked by a number of remote clients and
may see considerable variation in workload patterns over time. Each application
is associated with a SLO deadline by which it must respond to client requests.

\subsection{Fungible Application Development Workflow}

%\begin{figure}
%	\centering
%	\resizebox{\columnwidth}{!}{
%		\includegraphics{figures/fcc.pdf}
%	}
%	\caption{RPC processing for fungible compute contexts.}
%	\label{fig:fcc}
%\end{figure}

%Developers writing fungible applications must provide an implementation of the
%application logic for each hardware backend that they would like to target, and
%integrate it with a network processing library provided by \sys.

%Developers can then implement application logic for each target backend in an
%appropriate programming language (e.g., C++ for CPUs, SystemVerilog for FPGAs)
%and integrate a network processing pipeline.

To actually benefit from fungible computing, \sys requires that each application
can be accessed with the same network RPCs across multiple fungible compute
platforms. This means that developers must implement and maintain multiple
versions of their applications for each target backend and integrate them with
an \sys-provided RPC library.

While solving the single-source compilation challenge---a popular and on-going
research
topic~\autocite{auerbach2012_Compiler,canis2013_LegUp,circt_CIRCT,greaves2010_Designing,lattner2021_MLIR,tine_SingleSource,ringlein2020_Programming,villarreal2010_Designing}---is
out of scope for \sys, we believe this is still a reasonable requirement
because: (1)~good hardware development practices already lead developers to
build software co-simulation frameworks along with behavioural and functional
hardware models for better testing, making it easier to have a software
implementation~\autocite{li2020_Reproducible,moreau2019_Hardware,vega_LastLayer},
and (2)~if moving interactive applications from CPUs to FPGAs for higher
efficiency (a major target use case for \sys), it is likely that a CPU version
of the application code already exists and can be reused.

Alternatively, developers can use domain-specific compilation stacks such as for
machine
learning~\autocite{chen2018_TVM,noronha2018_LeFlow,sharma2016_Highlevel,zhang2018_DNNBuilder},
or high-level RTL compilers such as OpenCL~\autocite{stone2010_OpenCL},
LegUp~\autocite{canis2013_LegUp}, and High-Level
Synthesis~\autocite{cong2011_HighLevel} to compile high-level application
specifications to different hardware backends (with minimal changes). With the
explosion of domain-specific compilation techniques for multiple hardware
platforms~\autocite{huang2021_DSLs,lattner2021_MLIR,circt_CIRCT}, we expect
single-source compilation methods to become widespread over time. Developers
then only need to interface their automatically-generated applications with
\sys's RPC stack to ensure resource fungibility.

\subsection{System Overview}

\begin{figure}
	\centering
	\resizebox{0.9\columnwidth}{!}{
		\includegraphics{figures/design_overview/design.pdf}
	}
	\caption{\sys design overview.}
	\label{fig:design_overview}
\end{figure}

%Fungible computing requires hardware backends such as CPUs and FPGAs to provide
%a uniform control API for resource management, and a uniform application API to
%program against and execute applications.
%
%Fungible computing requires execution platforms to expose a uniform API to
%program, manage, and execute user applications.

\Cref{fig:design_overview} shows the high-level design of \sys.

To register a new application, clients must send a \emph{registration message}
to \sys's centralized \emph{orchestration gateway}. The registration message
provides application images (e.g., CPU binaries and FPGA bitstreams) and
specifies application constraints such as the SLO deadline (a constant multiple
of the average service time) and the maximum worker concurrency
limit~\autocite{amazonwebservices_AWSa}. Upon receipt, the gateway registers the
application by assigning it a unique \texttt{appID}, saves its binaries in the
\emph{image store}, and returns the \texttt{appID} and an invocation address
back to the client.

Clients can then use the \texttt{appID} to make application requests to the
gateway address. As the gateway receives client requests, it transparently
handles allocations by spinning \emph{fungible compute workers} up/down on a
disaggregated pool of \emph{hardware backends}. Backends which do not already
have an image in their \emph{image cache} pull one from image store before
spinning up a worker. Upon allocation, the gateway forwards client requests to
the worker by issuing RPC calls to its backend. Backends dispatch requests to
workers which process RPCs and return the result back to the gateway, which then
forwards it to the client as a response.

\subsection{Orchestration Gateway}

The gateway shares a design similar to existing serverless
frameworks~\autocite{openfaas_OpenFaaS, apache_OpenWhisk,jia2021_Nightcore},
with four key differences: (1)~it manages multiple types of fungible hardware
backends and provides orchestration primitives such as worker allocation,
autoscaling, and fault tolerance, (2)~it load balances incoming client requests
across allocated workers by invoking RPCs and returning results, (3)~it profiles
energy and performance metrics of application requests on these backends, and
(4)~it implements a scheduling policy that uses these profiles and attempts to
minimize the overall energy consumption while still meeting latency SLOs
(\Cref{sec:orchestration}).

\sys's centralized gateway is responsible for both control plane (application
registration, allocation) and data plane (scheduling) operations. It can handle
worker allocations on the request dispatch path, which lets it quickly adapt to
incoming load~\autocite{cloudflare_Eliminating}. This also enables it to scale
the number of allocated workers down to zero to save energy, and quickly scale
back up if new requests arrive.

%\begin{table}
%	\centering
%	\begin{tabular}{llll}
%		\toprule
%		API call        & Operation                      &   & \\
%		\emph{allocate} & allocate a compute context     &   & \\
%		deallocate      & deallocate a compute context   &   & \\
%		get\_metrics    & obtain perf and energy metrics
%		                &                                &     \\
%		\bottomrule
%	\end{tabular}
%	\caption{Control Plane API exposed by Backend Managers.}
%	\label{tab:control_plane_api}
%\end{table}

\subsection{Image Store}

The image store is a simple persistent store of application images for different
compute backends, and serves the appropriate image to workers in case they do
not have them locally upon warmup. It is similar to cloud storage services like
Amazon S3 used for AWS Lambda images~\autocite{amazonwebservices_Lambda}.

\subsection{Disaggregated Hardware Backends}

Hardware backends are shared, network-attached compute platforms that can run
one or more fungible compute workers. Backends are responsible for local
allocations and deallocations of compute workers, and for forwarding gateway
RPCs to workers by using the \texttt{workerID} field. Each backend consists of
three shared system components: (1)~a RPC / networking stack that facilitates
application I/O for the compute workers, (2)~a backend manager that exposes a
uniform control plane API to the orchestration gateway and helps monitor the
backend, and (3)~an image cache, that stores recent or popular application
images to speed up spin up times.

\sys currently supports two types of backends---CPUs and FPGAs---but can be
extended to other types. CPU backends run the backend manager on a dedicated
core and launch workers on other cores. FPGA backends have reconfigurable logic
directly connected to the network and have a split control and data plane for
backend managers. On the FPGA, they run a shell which provides uniform network
and memory I/O
interfaces~\autocite{caulfield2016_Cloudscale,korolija2020_OS,zhang2017_Feniks,tarafdar2019_Building},
and assume the existence of a lightweight control-plane CPU or over-the-network
reprogramming to spin up compute workers~\autocite{ringlein2019_System}.
Although disaggregation is not required as we show in~\Cref{sec:evaluation}, it
is preferable because it reduces resource stranding and improves efficiency by
enabling independent resource scaling [cite].

\subsection{Fungible Compute Workers}

To uniformly run the same application requests on multiple types of hardware, we
introduce the notion of \emph{fungible compute workers}, which are
hardware-agnostic execution environments with a programmable data plane.
Abstractly, each worker can be thought of as a function or library API with
common inputs and outputs, but with multiple implementations that allows
interoperability on different hardware backends. Worker are launched by backend
managers using an appropriate image from the image store/cache. Each worker has
a bounded queue of requests of configurable length and runs requests to
completion without preemption. Worker lifetimes are controlled fully by backend
managers.

%Fungible compute workers receive inputs from the underlying network stack which
%they transform and use as application inputs. Similarly, they transform
%application responses before sending them out onto the network.

%Network-attached FPGAs run the RPC stack
%directly inside the FPGA shell, while the backend manager is run on a small
%control-plane CPU that is used for FPGA reprogramming. However, the same API
%could be exposed by the backend manager entirely in hardware.

%%% FUTURE WORK (IDL, PCIe-attached FPGAs etc)

%The PCIe-attached FPGA may also have a CPU component of the
%application which is started similar to processes on CPU backends.
%\todo{how to integrate programmable RPC dataplane API into this story?}
%On CPUs and PCIe-attached FPGAs, both components run on a
%separate core on the host CPU. A small part of the backend manager runs
%inside the FPGA shell for PCIe-attached FPGAs, and is responsible for
%collecting metrics [whats-a-shell]

%\subsection{Programmable Data Plane}
%
%Fungible compute contexts expose a user-programmable data plane to specify the
%input and output interface to application logic. The data plane is programmed
%using an IDL and supports streaming and buffering data transmission modes for
%efficient application execution. We discuss each of these aspects below.

% Developers specify the application input and output schema
% using an Interface Definition Language (IDL) similar to Protobufs (Section X).
% For each supported hardware backend, the IDL compiler automatically generates
% function stubs and packet buffer serialization and deserialization code that
% sits on top of the networking stack to expose uniform I/O semantics to
% applications (\Cref{fig:fcc}).

%\subsubsection{Interface Definition Language}
%
%We build a Interface Definition Language (IDL), similar to Apache
%Thrift~\autocite{apache_Thrift} and Google Protobuf~\autocite{google_Protocol},
%that allows developers to define hardware-agnostic input and output message
%types and application interfaces. Crucially, unlike existing hardware RPC stacks
%that transfer data from FPGAs back to CPUs for application processing [dagger],
%our IDL can generate code for applications that run entirely on network-attached
%FPGAs.
%
%\Cref{fig:idl} shows a example of our IDL used to specify a simple
%image resizing application. We use a Protobuf-like syntax to define data types
%and declare the application type and interface.
%The  \texttt{resize} function takes as input an \texttt{Image} message
%containing a 128$\times$128 byte array and downscales it to a 32$\times$32 byte
%array which it returns as output to the caller.
%
%\begin{figure}[h]
%	\lstinputlisting[language=C++]{figures/struct.cpp}
%	\caption{Image resizing application specified using our IDL.}
%	\label{fig:idl}
%\end{figure}

%\lstnewenvironment{MyCode}
%{
%	\lstset{
%		language=C++,
%		%basicstyle=\fontfamily{fvm}\selectfont,
%		keywordstyle=\bfseries,
%		identifierstyle=\color{blue},
%		commentstyle=\color{ForestGreen},
%		%stringstyle=\fontfamily{fvs}\selectfont,
%		frame=single,showstringspaces=false,columns=flexible}
%} {}

%This interface definition gets compiled down into a C interface file for CPU
%backends and a Verilog module specification for hardware backends. Note that
%our current implementation does not support nested structures.
%
%\begin{figure}[h]
%	\begin{lstlisting}[language=C]
%char** resize(char pixels_i[128][128]);
%\end{lstlisting}
%	\caption{Generated C++ function interface}
%\end{figure}
%
%\begin{figure}[h]
%	\begin{lstlisting}[language=Verilog]
%module resize(
%	..., // clk, rst, etc.
%	input			startof_pixels_i,
%	input			endof_pixels_i,
%	input			valid_pixels_i,
%	input	[511:0] pixels_i,
%
%	output			startof_pixels_o,
%	output			endof_pixels_o,
%	output			valid_pixels_o,
%	output	[511:0] pixels_o
%);
%endmodule
%\end{lstlisting}
%	\caption{Generated SystemVerilog module \todo{fix this}}
%\end{figure}

% Code example

% IDL hardware block

%\subsubsection{Data Transmission Modes}
%
%Application inputs and outputs specified in the IDL can use either buffered or
%streaming data transmission modes.
%
%Buffered mode guarantees that the entire input data is
%available in the packet buffer before the application is invoked. The
%packet processing code generated from the IDL handles the data collection and
%buffering before invoking the application. Similarly, the buffered mode only
%sends a response once the application logic has finished processing and dumped
%its output into DRAM. While convenient, buffered transmission can slow down
%applications that can operate on partial data.
%
%Streaming mode provides data in the form of a stream to the application right
%away, and delegates the responsibility on performing data availability and
%bounds checks to the application. On the output side, it allows the
%developer to send data to the networking stack whenever desired. This offloads
%work to the developer to ensure that the right data semantics are being met,
%but can provide greater efficiency than the buffered case.
%
%FigX shows a SHA256 application that uses a stream of data blocks as input and
%provides a (buffered) hash as output. Note that a single RPC can use
%different data transmission modes for input and output.

%\begin{lstlisting}[language=C]
%rpc sha256(stream Block) returns (Hash);
%\end{lstlisting}

%\subsubsection{Network Function Interface}
%\pratyush{Should we include this to support network functions or just have
%	RPCs?}
%
%In addition to primitive data types and data arrays used to support RPC
%applications, our IDL also supports raw packets as input/output data types to
%applications. This enables developers to specify and build fungible network
%functions that can interact with packets at different layers of the networking
%stack [serverless-nf].
%We provide support for Ethernet, IP, and TCP packet packets and their headers
%by default. Alternatively, the developer may
%specify a custom packet schema that will be parsed by the underlying networking
%stack and passed to the application.
%
%\begin{lstlisting}[language=C]
%nf NAT(TCPHeader) forwards (TCPHeader);
%\end{lstlisting}

% We probably don't want to talk about isolation
%\subsection{Isolation}
%
%As fungible compute contexts target latency-sensitive computation in a
%shared environment, they must provide performance isolation and memory safety
%to applications. Each fungible compute context
%attempts to provide the abstraction of a predictable worker, which
%can then be used to compose predictable end-to-end systems [clockwork].
%
%\todo{what exactly can we provide for isolation?}
%Specifically, on CPUs, fungible compute contexts are run on separate cores with
%a pre-specified amount of memory to minimize interference. To avoid
%interference on the shared network stack and memory interfaces...
%
%FPGAs have the added benefit to be able to provide static, circuit-level
%isolation at compile time. However, they do not isolate shared interfaces such
%as the network and DRAM. FPGA contexts are run on separate
%partially-reconfigurable regions. To separate memory, we provide a uniform
%memory access interface to applications.


==> sections/discussion.tex <==
\section{Limitations and Discussion}
\label{sec:discussion}

\todo{keep?}
We highlight limitations of our modeling and analysis, and discuss potential future mitigations.

\smallskip
\noindent\textbf{Modeling Assumptions.}
Power states beyond busy and idle?
Stateful applications? 
Worker sharing?

\smallskip
\noindent\textbf{Scheduling.}
Pareto optimal scheduler with a knob?
Trade-off between repeated worker allocations and keeping workers idle?
Scarce workers and multiple applications?

\smallskip
\noindent\textbf{Reducing Spin-up Costs.}
\begin{itemize}[nosep]
	\item Partial reconfiguration
    \item Overlays
	\item Avalon-ST, Xilinx parallel interface
	\item Ethernet link training time
	\item Design a board that has an SRAM wired directly to the parallel
	      configuration interface instead of Flash
	\item Single ISA ML FPGAs~\autocite{zeng2020_Enabling}
    \item Yet, hybrid computing can still help improve overall datacenter utilization 
\end{itemize}

\smallskip
\noindent\textbf{Diverse Workers.}
GPUs also offer similar trade-offs as FPGAs; for example, it takes longer to start-up and load models on a GPU than on a CPU in NVIDIA Triton inference server.
We plan to evaluate other compute elements such as GPUs and ASICs in future work.


==> sections/implementation.tex <==
\section{Implementation}
\label{sec:implementation}

To test out a broad set of workloads and configurations, we also implemented a
discrete event simulator and workload generator in Cython/C++.

\todo{need this section?}

==> sections/system_model.tex <==
\section{System Model}
\label{sec:system_model}

We start by describing our target applications and hybrid platforms. Then, we survey target workloads and the trade-offs between FPGA and CPU workers.
\todo{this section feels oddly placed, how to move/rewrite?}

\subsection{Hybrid Platforms}

%Self-similarity roughly refers to similar (auto-correlated) variability at a wide range of timescales. 


\subsection{Workloads}

%Although maintaining multiple
%implementations may seem challenging, we note that there is a large--and
%growing--body of work on single source
%compilation~\autocite{zhang2022_HeteroGen,xiao2022_PLD,auerbach2012_Compiler,canis2013_LegUp,stone2010_OpenCL,huang2021_DSLs,circt_CIRCT,greaves2010_Designing,lattner2021_MLIR,tine_SingleSource,ringlein2020_Programming,villarreal2010_Designing}
%and domain-specific multi-backend
%compilation~\autocite{chen2018_TVM,noronha2018_LeFlow,sharma2016_Highlevel,zhang2018_DNNBuilder}
%which developers can benefit from. These tools can compile the same high-level
%application logic down to multiple hardware backends.


